FISHER: Gradient-Decoupled Hierarchical Multi-Task Learning for Fine-Grained Aquatic Species Recognition

Fine-grained recognition of aquatic species is challenging due to subtle morphological differences and long-tailed distributions, where ultra-rare species are underrepresented. A natural solution is to jointly model segmentation, morphological traits, and species classification within a multi-task learning (MTL) framework. However, existing MTL methods suffer from negative transfer caused by gradient conflicts between low-level dense tasks and high-level classification objectives, degrading fine-grained representations. To address this limitation, we identify gradient interference across hierarchical tasks as a fundamental bottleneck and propose FISHER, a gradient-decoupled hierarchical multi-task learning framework. FISHER aligns optimization with the biological hierarchy of aquatic species by enforcing a unidirectional information flow from segmentation to trait prediction and finally to species classification, while explicitly decoupling gradients across task boundaries. This design prevents high-level objectives from corrupting low-level morphological representations, effectively mitigating negative transfer while preserving the benefits of shared supervision. Furthermore, we introduce a prototypebased segmentation head with orthogonality regularization to encourage disentangled anatomical representations, and employ homoscedastic uncertainty weighting to dynamically balance task contributions during training. Our analysis shows that robust trait representations serve as a critical bridge for transferring knowledge to ultra-rare species. Extensive experiments on the Fish-Vista benchmark demonstrate that FISHER achieves 97.7% mAP for trait identification on unseen species and improves ultra-rare species classification accuracy by 13.4% over strong baselines, highlighting the effectiveness of gradient-decoupled hierarchical learning for long-tailed biodiversity recognition.

==> tables/clsnew.tex <==
\begin{table*}[!htbp]
\small
\centering
\setlength\tabcolsep{2.5pt} % Tăng khoảng cách cột nhẹ cho dễ nhìn
\renewcommand{\arraystretch}{1.1} % Tăng chiều cao dòng nhẹ
\resizebox{0.75\textwidth}{!}{
\begin{tabular}{lccccc}
    \toprule
        \textbf{Model} & \textbf{F1} & 
        \begin{tabular}[c]{@{}c@{}}\textbf{Major} \\ \textbf{Acc.}\end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}\textbf{Neutral} \\ \textbf{Acc.}\end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}\textbf{Minor} \\ \textbf{Acc.}\end{tabular} & 
        \begin{tabular}[c]{@{}c@{}}\textbf{Ultra-R} \\ \textbf{Acc.}\end{tabular} \\ 
    \midrule
    
    % --- General Backbones ---
    \textit{General Backbones} & & & & & \\
    \textbf{VGG-19} \cite{simonyan2014very} & 49.7 & 93.5 & 83.0 & 74.2 & 45.9 \\
    \textbf{ResNeXt-50} \cite{xie2017aggregated} & 44.4 & 91.4 & 78.3 & 69.8 & 39.1 \\ 
    \textbf{ViT-B16} \cite{ViT} & 48.3 & 88.7 & 82.3 & 73.3 & 43.4 \\
    \textbf{Swin-B-22k} \cite{swin} & 55.1 & 92.6 & 86.2 & 79.6 & 50.4 \\
    \textbf{MaxViT-T} \cite{maxvit} & 57.8 & 94.4 & 86.7 & 81.4 & 53.9 \\
    \midrule
    
    % --- Foundation Models ---
    \textit{Foundation Models (Linear Probe)} & & & & & \\
    \textbf{BioCLIP-LP} \cite{bioclip} & 38.2 & \colorbox{red!15}{75.5} & \colorbox{red!15}{65.2} & 61.3 & 31.1 \\
    \textbf{DINOv2-LP} \cite{oquab2023dinov2} & 53.1 & 89.9 & 78.0 & 76.0 & 47.0 \\
    \midrule
    
    % --- Specialized Methods ---
    \textit{Specialized Methods} & & & & & \\
    \textbf{INTR} \cite{paul2023simple} & \colorbox{red!35}{6.1} & 92.2 & 73.2 & \colorbox{red!35}{22.6} & \colorbox{red!35}{0.6} \\
    \textbf{TransFG} \cite{he2022transfg} & 50.3 & 94.5 & 86.6 & 75.5 & 45.3 \\
    \midrule
    
    % --- Ours ---
    \textit{Ours} & & & & & \\
    \textbf{MTLSwinB} (Parallel Baseline) & \colorbox{blue!15}{57.9} & 95.2 & \colorbox{blue!15}{89.0} & \colorbox{blue!15}{85.9} & 60.5 \\
    \textbf{ProtoMTL} & \colorbox{blue!15}{57.9} & \colorbox{blue!15}{95.4} & \colorbox{blue!35}{89.8} & 84.8 & 59.7 \\
    \textbf{GILLS} (Proposed) & \colorbox{blue!35}{60.8} & \colorbox{blue!35}{95.5} & \colorbox{blue!15}{89.0} & \colorbox{blue!35}{86.2} & \colorbox{blue!35}{63.8} \\
    \bottomrule
\end{tabular}
}
\caption{Comparison of classification performance (in \%). We select representative baselines from CNNs, Transformers, Foundation Models, and FGVC methods. Results are color-coded as \colorbox{blue!35}{Best}, \colorbox{blue!15}{Second best}, \colorbox{red!35}{Worst}, \colorbox{red!15}{Second worst}.}
\label{tab:classification}
\end{table*}

==> tables/consistency.tex <==

\begin{table}[t]
\centering
\caption{Internal consistency of $\FISHER$'s hierarchical predictions on the
classification test set. \emph{Species$\to$Trait}: fraction of
samples where the predicted species agrees with the predicted trait; \emph{Seg$\to$Trait}:
fraction where the segmented anatomical part agrees with the predicted trait}
\label{tab:consistency}
\small
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{8pt}
\begin{tabular}{lcc}
\toprule
Trait & Species$\to$Trait (\%) & Seg$\to$Trait (\%) \\
\midrule
Adipose Fin & 99.86 & 97.06 \\
Pelvic Fin  & 99.99 & 95.10 \\
Barbel      & 99.67 & 93.73 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/cub.tex <==
\begin{table}[H]
\centering
\ph{\caption{Cross-domain validation on \textbf{CUB-LT} with a $500{:}1$ imbalance factor and $96$ tail classes. All variants use the same Swin-B backbone and three-head architecture, differing only in gradient flow. Results are mean$\pm$std over $5$ seeds}}
\label{tab:cub_lt}
\renewcommand{\arraystretch}{1.2}
\resizebox{\columnwidth}{!}{%
\ph{\begin{tabular}{l c c c}
\toprule
Method & Top-1 (\%) & Tail Acc. (\%) & Attr. mAP (\%) \\
\midrule
Single-Task            & $57.96${\scriptsize$\pm1.79$} & $44.57${\scriptsize$\pm1.18$} & -- \\
Parallel MTL (Connected) & $57.23${\scriptsize$\pm1.80$} & $42.73${\scriptsize$\pm2.05$} & $25.24${\scriptsize$\pm0.46$} \\
$\FISHER$ (Detached)   & $58.64${\scriptsize$\pm1.98$} & $45.60${\scriptsize$\pm1.32$} & $\mathbf{26.88}${\scriptsize$\pm0.43$} \\
\bottomrule
\end{tabular}}%
}
\vspace{-1em}
\end{table}

==> tables/efficiency.tex <==

\begin{table}[H]
\centering
\caption{Efficiency comparison at Fish-Vista scale on a single GPU NVIDIA RTX~4070)}
\label{tab:efficiency}
\renewcommand{\arraystretch}{1.15}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l c c c c}
\toprule
Model & Params (M) & GFLOPs & Latency$_{b=1}$ (ms) & Throughput$_{b=32}$ (img/s) \\
\midrule
RegNetY-4G            & 24.3  & 8.0  & 3.08 & 1083.0 \\
ResNeXt-50            & 31.8  & 8.6  & 1.53 & 855.8 \\
MaxViT-T              & 32.6  & 10.7 & 6.61 & 442.1 \\
ViT-B/16              & 89.1  & 33.7 & 4.16 & 384.2 \\
Swin-B (single-task)  & 91.2  & 30.4 & 5.15 & 304.6 \\
VGG-19                & 157.3 & 39.3 & 5.63 & 447.2 \\
\midrule
Parallel MTL (Connected)$^\dagger$ & 96.8 & 39.8 & 6.28 & 261.9 \\
$\FISHER$ (Detached)$^\dagger$     & 96.8 & 39.8 & 6.28 & 261.9 \\
\bottomrule
\end{tabular}%
}
\vspace{-1em}
\end{table}

==> tables/fishvista_stats.tex <==
% =====================================================================
%  Fish-Vista frequency-stratified class distribution.
%  Computed from master_dataset.csv, stratified by NUMBER OF TRAINING
%  SAMPLES (counts within the `train` split only, 47,595 images) --
%  the same basis as the classification performance groups.
%  697 of 4,316 species have ZERO training images (test_ood only) and
%  are excluded here (disclosed in footnote), not folded into Ultra-Rare.
% =====================================================================
\begin{table}[H]
\centering
\caption{Frequency-stratified class distribution of Fish-Vista~\cite{Fishvista},
computed on the $47{,}595$-image \textit{train} split: \textit{Majority} ($\ge500$), \textit{Neutral}
($100$--$499$), \textit{Minority} ($10$--$99$), \textit{Ultra-Rare} ($<10$) images}
\label{tab:fishvista_stats}
\renewcommand{\arraystretch}{1.15}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l r r r r}
\toprule
Group & \#Classes & \% Classes & \#Train Images & \% Images \\
\midrule
Majority ($\ge500$)     & 20    & 0.6\%  & 25{,}246 & 53.0\% \\
Neutral ($100$--$499$)  & 35    & 1.0\%  & 7{,}278  & 15.3\% \\
Minority ($10$--$99$)   & 331   & 9.1\%  & 7{,}458  & 15.7\% \\
Ultra-Rare ($<10$)      & 3{,}233 & 89.3\% & 7{,}613  & 16.0\% \\
\midrule
Total (trained species) & 3{,}619 & 100\% & 47{,}595 & 100\% \\
\bottomrule
\end{tabular}%
}
\vspace{-1em}
\end{table}

==> tables/grad.tex <==
\begin{table*}[H]
\centering
\caption{Ablation to verify the effectiveness of our architectural detachment for multi-task learning. \textbf{Ultra-R} denotes accuracy on the hardest Ultra-Rare species subset ($<10$ samples). All experimental results are extracted by using the Swin-B backbone. GradNorm was re-tuned across learning-rate and $\alpha$ settings; the reported figures use the best configuration.}
\label{tab:gradient_conflict}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{l l c c c c}
\toprule
Method & Optimization Strategy & Species F1 (\%) & Ultra-R Acc. (\%) & Trait OOD mAP (\%) & Seg mIoU (\%) \\
\midrule
Standard MTL & Naive Sum ($\sum \mathcal{L}_i$) & 53.8 & 56.1 & 88.8 & 76.9 \\
MTL + UW \cite{8578879} & Uncertainty Weighting & 57.8 & 60.4 & 92.7 & \textbf{80.4} \\
MTL + GradNorm \cite{pmlr-v80-chen18a} & Gradient Normalization & 56.9 & 58.1 & 79.7 & 75.6 \\
MTL + PCGrad \cite{yu2020gradient} & Gradient Projection & 58.1 & 59.6 & 80.2 & 78.3 \\
\midrule
$\FISHER$ & Gradient Detachment & \textbf{60.8} & \textbf{63.8} & \textbf{97.7} & 79.8 \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/lt_baselines.tex <==

\begin{table}[H]
\centering
\caption{Comparison with specialized long-tailed methods on Fish-Vista.
All long-tailed rows share $\FISHER$'s exact Swin-B-22k backbone, training
schedule, and are \emph{single-task}
classifiers differing only in the loss/sampling strategy}
\label{tab:lt_baselines}
\renewcommand{\arraystretch}{1}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l c c c c c}
\toprule
Method & Macro-F1 & Majority & Neutral & Minority & Ultra-Rare \\
\midrule
\multicolumn{6}{l}{\textit{Long-tailed methods (Swin-B backbone, single-task)}} \\
Balanced-Softmax         & 53.36 &  95.97 & 89.07 & 83.82 & 59.50 \\
LDAM-DRW                 & 52.61 & 96.03 & 89.07 & 82.93 & 56.95 \\
cRT (Decoupling)         & \underline{54.92} & 96.12 & \underline{89.66} & \underline{84.00} & \underline{59.98} \\
\midrule
\multicolumn{6}{l}{\textit{Reference (published, Table~3)}} \\
Swin-B                   & 55.10 & 92.6 & 86.2 & 79.6 & 50.4 \\
\textbf{$\FISHER$ (ours)} & \textbf{60.80} & 95.5 & 89 & 86.2 & \textbf{63.80} \\


\bottomrule
\end{tabular}%
}
\vspace{-1em}
\end{table}

==> tables/seed_robustness.tex <==
\begin{table}[t]
\centering
\caption{Multi-seed robustness on Fish-Vista \\ (Mean$\pm$std over $3$ random seeds)}
\label{tab:seed_robustness}
\renewcommand{\arraystretch}{1.2}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l c c c c}
\toprule
Metric & FISHER best & \shortstack{$\FISHER$\\(mean$\pm$std)} &
\shortstack{Parallel MTL\\(mean$\pm$std)} & \shortstack{Swin-B single-task\\(mean$\pm$std)} \\
\midrule
Species F1 (macro)        & 60.8  & $\mathbf{60.20\pm0.56}$ & $58.09\pm0.86$ & $54.55\pm0.65$ \\
Ultra-Rare accuracy       & 63.8  & $\mathbf{63.20\pm0.55}$ & $60.57\pm0.99$ & $49.80\pm0.90$ \\
Segmentation mIoU         & 79.8  & $\mathbf{80.01\pm0.31}$ & $79.15\pm0.59$ & -- \\
Trait mAP (In-Species)    & 99.11 & $99.38\pm0.23$          & $99.48\pm0.16$ & -- \\
Trait mAP (Leave-Out)     & 97.72 & $\mathbf{95.27\pm2.16}$ & $88.65\pm4.99$ & -- \\
Trait mAP (Manual)        & 79.53 & $\mathbf{80.23\pm0.90}$ & $75.71\pm2.11$ & -- \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/table_ablation_main.tex <==
\begin{table*}[ht]
\centering

\caption{Ablation Study for Comprehensive Structural \& loss. Results Are Highlighted as \colorbox{blue!35}{Best}, \colorbox{blue!15}{Second best}, \colorbox{red!35}{Worst}, \colorbox{red!15}{Second worst}}
\label{tab:structural_ablation_full}

\resizebox{0.93\textwidth}{!}{%
\begin{tabular}{llccccc} 
\toprule
Variant & Configuration / Mechanism & Species F1 & Ultra-Rare Acc. & OOD Trait mAP & Seg mIoU & Barbel IoU \\ 
\midrule

% SECTION A
\multicolumn{7}{l}{\textbf{Scenario 1. }\textit{Component Ablation (Removing Modules)}} \\
Species Only & Species Only & \colorbox{red!15}{55.1} & \colorbox{red!35}{50.4} & -- & -- & -- \\
No Segmentation & Trait $\to$ Species & \colorbox{red!35}{54.7} & \colorbox{red!15}{57.7} & 94.2 & -- & -- \\
No Trait & Seg $\to$ Species & 57.1 & 60.0 & -- & 78.5 & \colorbox{red!15}{27.8} \\
\midrule

% SECTION B
\multicolumn{7}{l}{\textbf{Scenario 2. }\textit{Order \& Connectivity (Changing Topology)}} \\
Standard MTL & Parallel (Shared Backbone) & 57.8 & 60.4 & 92.7 & \colorbox{blue!35}{80.4} & \colorbox{blue!35}{34.5} \\
Reverse Order & Species $\to$ Trait $\to$ Seg ($\Downarrow$) & 58.5 & \colorbox{blue!15}{62.8} & 91.5 & \colorbox{blue!15}{80.1} & \colorbox{blue!15}{33.4} \\
Fully Connected & Seg $\to$ Trait $\to$ Species ($\Uparrow$) & \colorbox{blue!15}{60.1} & 61.4 & 94.1 & \colorbox{red!15}{78.3} & 28.9 \\
\midrule

% SECTION C
\multicolumn{7}{l}{\textbf{Scenario 3. }\textit{Partial Detachment (Negative Transfer)}} \\
Partial A (Seg Connect) & Seg $\to$ Trait $\parallel$ Species & 59.8 & 60.1 & \colorbox{red!35}{86.4} & 79.0 & 31.3 \\
Partial B (Trait Connect) & Seg $\parallel$ Trait $\to$ Species & 59.9 & 61.1 & \colorbox{red!15}{87.4} & 79.5 & 30.7 \\
\midrule

% SECTION D
\multicolumn{7}{l}{\textbf{Scenario 4. }\textit{Loss \& Weighting (Detached Architecture)}} \\
Base Detached & w/o UW and Ortho. Losses & 58.1 & 61.5 & \colorbox{blue!15}{95.7} & 79.2 & 32.6 \\
+ Uncertainty & w/ UW Only & 55.7 & 59.6 & 95.4 & \colorbox{red!35}{77.7} & \colorbox{red!35}{27.3} \\
+ OrthoLoss & w/ Orthogonal Loss Only & 58.1 & 62.2 & 94.5 & 79.1 & 31.9 \\
\midrule

% FINAL ROW
\rowcolor{blue!5} 
$\FISHER$ (Ours) & Detached + UW + Ortho. Losses & \colorbox{blue!35}{60.8} & \colorbox{blue!35}{63.8} & \colorbox{blue!35}{97.7} & 79.8 & 32.9 \\ 
\bottomrule
\end{tabular}
} \vspace{-1.0em}
\end{table*}

==> tables/table_classification.tex <==
\begin{table}[]
\small
\centering
\caption{Comparison of classification performance (in \%). Results are color-coded as \colorbox{blue!35}{Best}, \colorbox{blue!15}{Second best}, \colorbox{red!35}{Worst}, \colorbox{red!15}{Second worst} (excluding Zero-Shot methods \textbf{(ZS)}).}
\setlength\tabcolsep{1.5pt}
\renewcommand{\arraystretch}{1}
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{lccccc}
    \toprule
        
        \fontsize{9.2pt}{10}\selectfont\textbf{Model} & \fontsize{9pt}{10}\selectfont\textbf{F1} & \begin{tabular}[c]{@{}c@{}}{\fontsize{9pt}{10}\selectfont\textbf{Major}} \\
        {\fontsize{9pt}{10}\selectfont\textbf{Acc.}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\fontsize{9pt}{10}\selectfont\textbf{Neutral}} \\ {\fontsize{9pt}{10}\selectfont\textbf{Acc.}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\fontsize{9pt}{10}\selectfont\textbf{Minor}} \\ {\fontsize{9pt}{10}\selectfont\textbf{Acc.}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\fontsize{9pt}{10}\selectfont\textbf{Ultra-R}} \\
        {\fontsize{9pt}{10}\selectfont\textbf{Acc.}} \end{tabular}\\ \midrule
        \fontsize{8.5pt}{10}\textbf{VGG-19} \cite{simonyan2014very} & 49.7 & 93.5 & 83.0 & 74.2 & 45.9 \\
        % \textbf{ResNet-34} \cite{resnet} & 35.6 & 89.9 & 68.4 & 60.9 & 30.7 \\
        % \textbf{Inception-v3} \cite{inceptionv3} & 40.2 & 90.0 & 77.7 & 67.7 & 34.5 \\ 
        \fontsize{8.5pt}{10}\textbf{ResNeXt-50} \cite{xie2017aggregated} & 44.4 & 91.4 & 78.3 & 69.8 & 39.1 \\  
        \fontsize{8.5pt}{10}\textbf{RegNetY-4G} \cite{radosavovic2020designing} & 43.7 & 89.8 & 77.4 & 68.5 & 38.5 \\ 
        % \textbf{EfficientNetV2} \cite{tan2021efficientnetv2} & 34.3 & 89.0 & 75.0 & 62.3 & 28.5 \\ 
        \midrule
        \fontsize{8.5pt}{10}\textbf{ViT-B16} \cite{ViT} & 48.3 & 88.7 & 82.3 & 73.3 & 43.4 \\
        % \textbf{ViT-B32} \cite{ViT} & 45.2 & 86.9 & 75.8 & 66.6 & 41.8 \\
        % \textbf{DeiT-s} & 46.2 & 91.7 & 76.8 & 72.3 & 40.8 \\
        \fontsize{8.5pt}{10}\textbf{Swin-B-22k} \cite{swin} & 55.1 & 92.6 & 86.2 & 79.6 & 50.4 \\
        \fontsize{8.5pt}{10}\textbf{CvT-13} \cite{cvt} & 49.3 & 92.0 & 83.3 & 73.5 & 44.7 \\
        % \textbf{Mobile-ViT-xs} \cite{mehta2021mobilevit} & 49.0 & 92.2 & 85.9 & 74.1 & 43.7 \\
        % \textbf{Mobile-ViT-v2} \cite{mehta2022separable} & 42.7 & 91.4 & 80.8 & 66.8 & 37.6 \\ 
        \fontsize{8.5pt}{10}\textbf{MaxViT-T} \cite{maxvit} & 57.8 & 94.4 & 86.7 & 81.4 & 53.9 \\
        \fontsize{8.5pt}{10}\textbf{PVT-v2-b0} \cite{wang2022pvt} & 51.0 & 92.0 & 83.4 & 75.7 & 45.8 \\
        \midrule
        \fontsize{8.5pt}{10}\textbf{BioCLIP-ZS} \cite{bioclip} & 4.6 & 1.1 & 1.4 & 10.2 & 5.6 \\
        \fontsize{8.5pt}{10}\textbf{CLIP-ZS} \cite{clip} & 0.1 & 0.0 & 0.3 & 0.4 & 0.2 \\
        \midrule
        
        \fontsize{8.5pt}{10}\textbf{BioCLIP-LP} \cite{bioclip} & 38.2 & \colorbox{red!15}{75.5} & \colorbox{red!15}{65.2} & 61.3 & 31.1 \\
        
        \fontsize{8.5pt}{10}\textbf{CLIP-LP} \cite{clip} & \colorbox{red!15}{25.4} & \colorbox{red!35}{55.9} & \colorbox{red!35}{49.8} & \colorbox{red!15}{46.7} & \colorbox{red!15}{20.9} \\

        \fontsize{8.5pt}{10}\textbf{DINOv2-LP} \cite{oquab2023dinov2} & 53.1 & 89.9 & 78.0 & 76.0 & 47.0 \\
        
        \midrule
        \fontsize{8.5pt}{10}\textbf{INTR} \cite{paul2023simple} & \colorbox{red!35}{6.1} & 92.2 & 73.2 & \colorbox{red!35}{22.6} & \colorbox{red!35}{0.6} \\
        \fontsize{8.5pt}{10}\textbf{TransFG} \cite{he2022transfg} & 50.3 & 94.5 & 86.6 & 75.5 & 45.3 \\ \midrule
        
        \fontsize{8.5pt}{10}\textbf{MTLSwinB} & \colorbox{blue!15}{57.9} & 95.2 & \colorbox{blue!15}{89.0} & \colorbox{blue!15}{85.9} & 60.5 \\
        
        % \fontsize{8.5pt}{10}\textbf{ProtoMTL (Ours)} & \colorbox{blue!15}{57.9} & \colorbox{blue!15}{95.4} & \colorbox{blue!35}{89.8} & 84.8 & 59.7 \\
        
        \fontsize{8.5pt}{10}\textbf{AquaDeHi} & 57.5 & 94.9 & \colorbox{blue!15}{89.0} & 84.1 & \colorbox{blue!15}{61.4} \\
        
        \fontsize{8.5pt}{10}\textbf{AquaDeHi$^\dagger$} & \colorbox{blue!35}{60.8} & \colorbox{blue!35}{95.5} & \colorbox{blue!15}{89.0} & \colorbox{blue!35}{86.2} & \colorbox{blue!35}{63.8} \\
        \bottomrule
    \end{tabular}
}

\label{tab:classification}
\end{table}

==> tables/table_implementation.tex <==
\begin{table}[]
\centering
\caption{Implementation Details and Hyperparameter Settings}
\label{tab:implementation_details}
\resizebox{\columnwidth}{!}{
% Thay đổi quan trọng nhất ở đây: {lc} thay vì {l|c}
\begin{tabular}{lc} 
\toprule
Configuration & Value/Setting \\
\midrule

% Mục 1
\multicolumn{2}{l}{\textit{Optimization Setup}} \\
\midrule
Optimizer & AdamW \\
Learning rate & $1 \times 10^{-4}$ \\
Weight decay & $0.01$ \\
Batch size & 32 \\
Training epochs & 50 \\ 
LR scheduler & Cosine annealing \\
Warmup epochs & 5 \\
\midrule

% Mục 2
\multicolumn{2}{l}{\textit{Model Architecture}} \\
\midrule
Backbone & Swin-Base (ImageNet-22k) \\
Input size & $224 \times 224$ \\
Prototype temperature ($\tau$) & 0.1 \\
Number of prototypes & 10 (Background + 9 Traits) \\
\midrule

% Mục 3
\multicolumn{2}{l}{\textit{Loss Coefficients}} \\
\midrule
Orthogonality Weight ($\lambda_{ortho}$) & 0.5 \\
Label Smoothing ($\epsilon$) & 0.1 \\ 
\bottomrule
\end{tabular}
} \vspace{-1.0em}
\end{table}

==> tables/table_segmentation.tex <==
\begin{table*}[!htbp]
\small
\centering
\caption{\small{Segmentation performance comparison (mIoU in \%) including Input Size. Results are color-coded as \colorbox{blue!35}{Best}, \colorbox{blue!15}{Second best}, \& \colorbox{red!35}{Worst} (excluding Zero-Shot).}}
\setlength\tabcolsep{2.5pt}
\renewcommand{\arraystretch}{1.1}
\resizebox{0.80\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multirow{2.5}{*}{\textbf{Model}} & \multirow{2.5}{*}{\textbf{Size}} & \multirow{2.5}{*}{\textbf{mIoU}} & \multicolumn{10}{c}{\textbf{Trait-wise IoU}} \\
\cmidrule(lr){4-13}
 & & & \textit{BG} & \textit{Head}  & \textit{Eye} & \textit{Dorsal} & \textit{Pect.} & \textit{Pelvic} & \textit{Anal} & \textit{Caudal} & \textit{Adip.} & \textit{Barbel}
    \\
    \midrule
        \fontsize{8.5pt}{10}\selectfont\textbf{PSPNet} \cite{zhao2017pspnet} & \multirow{7}{*}{\textbf{$320\times320$}} & \colorbox{red!35}{73.8} & \colorbox{red!35}{94.6} & \colorbox{red!35}{84.3} & \colorbox{red!35}{77.7} & \colorbox{red!35}{85.1} & \colorbox{red!35}{67.1} & 80.5 & \colorbox{red!35}{83.0} & \colorbox{red!35}{88.7} & \colorbox{red!35}{56.9} & 20.1 \\ 
        \fontsize{8.5pt}{10}\selectfont \textbf{DeepLabV3} \cite{chen2017rethinking}&  & 74.9 & 95.0 & 85.4 & 78.1 & 86.0 & 71.2 & 83.0 & 85.3 & 88.8 & 58.1 & 18.2 \\ 
        \fontsize{8.5pt}{10}\selectfont \textbf{DeepLabV3+} \cite{deeplabv3plus2018} &  & 77.0 & 95.4 & 86.0 & 79.1 & 88.1 & 71.0 & 84.7 & 86.2 & 89.9 & 66.1 & 23.7 \\ 
        \fontsize{8.5pt}{10}\selectfont \textbf{UNet} \cite{ronneberger2015u}&  & 77.5 & 95.6 & 86.2 & 79.9 & 88.2 & 70.6 & \colorbox{blue!15}{84.8} & 86.6 & 90.8 & \colorbox{blue!15}{69.7} & 22.3 \\ 
        \fontsize{8.5pt}{10}\selectfont \textbf{Semantic FPN} \cite{kirillov2019panoptic}&  & 77.6 & 95.5 & 86.1 & 79.2 & 88.2 & 71.4 & \colorbox{blue!35}{85.0} & 86.4 & 90.3 & 67.6 & 26.3 \\ 
        \fontsize{8.5pt}{10}\selectfont \textbf{Mask2Former} \cite{cheng2021per}&  & \colorbox{blue!15}{81.6} & 95.5 & 86.4 & 79.1 & 87.6 & 74.2 & \colorbox{red!35}{76.1} & 84.7 & 88.8 & 59.6 & \colorbox{red!35}{0.0} \\ 
        \fontsize{8.5pt}{10}\selectfont \textbf{YOLOv8} \cite{varghese2024yolov8} &  & \colorbox{blue!35}{83.1} & \colorbox{blue!15}{96.8} & 84.5 & 83.1 & 88.0 & \colorbox{blue!35}{78.0} & 77.5 & 85.6 & 89.6 & 66.8 & 26.7 \\ 
        \midrule
        
        \fontsize{8.5pt}{10}\selectfont \textbf{MTLSwinB} & \multirow{1}{*}{\textbf{$224\times224$}} & 80.4 & 96.7 & 87.8 & 82.7 & 91.5 & 73.5 & 82.9 & 88.5 & \colorbox{blue!15}{92.9} & \colorbox{blue!35}{72.7} & \colorbox{blue!15}{34.5} \\ 
        % \fontsize{8.5pt}{10}\selectfont \textbf{ProtoMTL} &  & 79.7 & 96.7 & 88.0 & 82.5 & 91.4 & 73.3 & 83.3 & 88.8 & \colorbox{blue!15}{92.9} & 67.1 & 32.6 
        \midrule
        \fontsize{8.5pt}{10}\selectfont \multirow{2}{*}{\textbf{AquaDeHi$^\dagger$}} & $224\times224$ & 79.8 & \colorbox{blue!15}{96.8} & \colorbox{blue!15}{88.3} & \colorbox{blue!15}{83.2} & \colorbox{blue!15}{91.6} & 74.0 & 83.0 & \colorbox{blue!15}{89.0} & \colorbox{blue!15}{92.9} & 66.8 & 32.9 \\
        & $320\times320$ & 81.4 & \colorbox{blue!35}{97.0} & \colorbox{blue!35}{88.9} & \colorbox{blue!35}{85.8} & \colorbox{blue!35}{92.4} & \colorbox{blue!15}{76.5} & 84.3 & \colorbox{blue!35}{89.4} & \colorbox{blue!35}{93.3} & \colorbox{blue!15}{69.7} & \colorbox{blue!35}{36.3} \\
        \midrule
        
        \fontsize{8.5pt}{10}\selectfont \textbf{MOLMO + SAM} \cite{deitke2024molmo} & - & 39.1 & 85.3 & 37.4 & 29.8 & 50.3 & 29.7 & 38.5 & 36.1 & 83.4 & 0.4 & 0.6 \\ 
        \bottomrule
    \end{tabular}
    }

\label{tab:segmentation}
\end{table*}

==> tables/table_traits_inspecies.tex <==
\begin{table*}[h]
\centering
\caption{Trait identification results on mainstream visual models using the \textbf{in-species test set}. Results are color-coded as \colorbox{blue!35}{Best}, \colorbox{blue!15}{Second best}, \colorbox{red!35}{Worst}, \colorbox{red!15}{Second worst}.}
\renewcommand{\arraystretch}{0.9}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccccc}
\toprule
\multirow{2}{*}{{Model}} & \multicolumn{5}{c}{{Average Precision}} & \multicolumn{4}{c}{{F1@0.5}} & \multicolumn{4}{c}{{F1@optimal threshold}} \\ 
\cmidrule(lr){2-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
 & mAP & Adip & Pelv & Barb & Dors & Adip & Pelv & Barb & Dors & Adip & Pelv & Barb & Dors \\ \midrule
VGG-19 & 87.06 & 95.09 & 61.85 & 96.21 & 95.07 & 92.61 & 68.28 & 94.62 & 93.17 & 93.69 & 80.85 & 94.7 & 93.28 \\
ResNet-18 & 87.85 & 96.56 & 65.96 & 95.16 & 93.73 & 91.26 & 78.95 & 93.7 & 91.16 & 94.47 & 79.01 & 94.07 & 92.18 \\
ResNet-34 & 91.77 & 95.71 & 80.73 & 95.53 & 95.1 & 94.42 & 72.4 & 94.64 & 92.96 & 94.41 & 88.84 & 94.72 & 92.78 \\
Inception-v3 & \colorbox{red!15}{77.0} & 93.08 & 52.4 & \colorbox{red!35}{86.03} & \colorbox{red!35}{76.47} & \colorbox{red!35}{87.45} & 77.67 & \colorbox{red!15}{88.93} & \colorbox{red!35}{83.53} & 93.16 & 78.48 & \colorbox{red!35}{88.69} & \colorbox{red!35}{84.95} \\
ResNext-50 & 91.44 & 98.53 & 74.64 & 97.03 & 95.54 & 96.07 & 86.56 & 96.32 & 94.09 & 96.9 & 85.23 & 96.45 & 94.99 \\
MobileNet-v3 & 90.49 & 96.34 & 73.79 & 96.33 & 95.51 & 94.38 & 83.73 & 95.19 & 93.69 & 94.58 & 84.26 & 95.14 & 94.73 \\
RegNet-Y & 89.51 & 95.54 & 73.06 & 95.45 & 94.0 & 94.62 & 82.28 & 94.86 & 94.12 & 94.69 & 81.6 & 94.77 & 94.04 \\
EfficientNet-v2 & 95.96 & 99.7 & 86.41 & 98.43 & 99.3 & 98.13 & 90.69 & 97.29 & 98.04 & 98.48 & 92.22 & 97.23 & 98.28 \\
ConvNext-Base & 97.46 & 99.54 & 92.33 & 98.67 & 99.32 & 98.62 & 92.31 & \colorbox{blue!15}{98.28} & 98.46 & 98.62 & 95.93 & \colorbox{blue!15}{98.19} & 98.45 \\
\midrule
ViT-B-16 & 86.95 & 92.93 & 67.7 & 93.29 & 93.89 & 91.51 & 66.75 & 92.41 & 92.57 & \colorbox{red!15}{91.71} & 81.23 & 92.14 & 92.68 \\
ViT-B-32 & 81.44 & \colorbox{red!35}{89.79} & 59.81 & \colorbox{red!15}{89.18} & \colorbox{red!15}{86.97} & \colorbox{red!15}{88.13} & \colorbox{red!35}{64.63} & \colorbox{red!35}{88.48} & \colorbox{red!15}{86.57} & \colorbox{red!35}{90.08} & 79.07 & \colorbox{red!15}{89.46} & \colorbox{red!15}{87.91} \\
DEiT-distilled & 93.74 & 97.61 & 82.85 & 97.02 & 97.48 & 95.5 & 76.11 & 94.93 & 96.12 & 95.72 & 86.88 & 95.76 & 96.47 \\
SWIN-B & 92.02 & 96.64 & 76.98 & 97.35 & 97.11 & 94.99 & 82.12 & 95.69 & 95.46 & 95.28 & 86.78 & 95.76 & 95.76 \\
SWIN-B-22k & 95.21 & 98.05 & 86.94 & 97.55 & 98.28 & 95.95 & 86.37 & 96.07 & 96.47 & 96.12 & 91.29 & 96.13 & 96.62 \\
CVT-13 & 83.61 & 93.22 & \colorbox{red!15}{49.56} & 96.21 & 95.43 & 92.92 & 71.72 & 94.47 & 94.08 & 93.37 & \colorbox{red!15}{78.1} & 94.47 & 94.61 \\
Mobile-ViT-xs & \colorbox{red!35}{75.12} & \colorbox{red!15}{90.57} & \colorbox{red!35}{25.66} & 93.78 & 90.5 & 91.94 & \colorbox{red!15}{65.17}   & 93.84 & 91.21 & 92.7 & \colorbox{red!35}{66.94} & 94.25 & 90.96 \\
Mobile-ViT-v2 & 86.3 & 95.21 & 62.3 & 95.29 & 92.4 & 92.81 & 70.38 & 94.72 & 91.66 & 93.28 & 78.25 & 94.38 & 92.32 \\
MaxViT-t & 95.49 & 98.33 & 86.44 & 98.88 & 98.3 & 96.87 & 87.71 & 97.91 & 97.77 & 97.06 & 91.99 & 97.74 & 97.68 \\
PVT-v2 & 96.48 & 98.84 & 90.85 & 97.75 & 98.49 & 97.61 & 84.15 & 96.94 & 97.58 & 97.62 & 91.63 & 97.15 & 97.92 \\
\midrule
Q2L (R34-22k SH) & 97.78 & 99.47 & 93.91 & 98.47 & 99.26 & 97.65 & 97.36 & 97.35 & 98.27 & 97.9 & 95.1 & 97.73 & 98.45 \\
Q2L (R34-22k MH) & 97.22 & 99.4 & 91.92 & 98.38 & 99.17 & 98.05 & 96.65 & 97.43 & 98.39 & 98.36 & 96.03 & 97.61 & 98.62 \\
Q2L (SwinB-22k SH) & 98.32 & 99.81 & 94.94 & \colorbox{blue!15}{99.0} & 99.53 & \colorbox{blue!35}{99.09} & 97.36 & 97.82 & \colorbox{blue!35}{99.19} & \colorbox{blue!15}{98.93} & 95.66 & 98.03 & \colorbox{blue!15}{99.06} \\
Q2L (SwinB-22k MH) & 98.32 & \colorbox{blue!15}{99.82} & 94.91 & 98.94 & \colorbox{blue!35}{99.61} & 98.73 & 98.04 & \colorbox{blue!35}{98.38} & \colorbox{blue!15}{99.02} & 98.93 & 96.82 & \colorbox{blue!35}{98.35} & \colorbox{blue!35}{99.23} \\ \midrule
\textbf{MTLSwinB} & \colorbox{blue!15}{99.38} & 99.75 & \colorbox{blue!15}{99.99} & 98.47 & 99.29 & 98.57 & \colorbox{blue!35}{99.97} & 97.19 & 98.21 & 98.87 & \colorbox{blue!15}{99.97} & 97.15 & 98.43 \\
% \textbf{ProtoMTL (Ours)} & 99.34 & \colorbox{blue!35}{99.94} & 99.97 & 98.26 & 99.18 & 98.58 & \colorbox{blue!35}{99.97} & 97.12 & 98.60 & 98.58 & \colorbox{blue!15}{99.97} & 97.62 & 98.59 \\
\textbf{AquaDeHi} & \colorbox{blue!35}{99.54} & 99.48                      & \colorbox{blue!35}{100.0} & \colorbox{blue!35}{99.10} & \colorbox{blue!15}{99.60} & 97.90 & \colorbox{blue!35}{99.97} & 97.28 & 98.11 & 97.90 & \colorbox{blue!15}{99.97} & 97.25 & 97.78 \\
\textbf{AquaDeHi$^\dagger$}  & 99.11 & 99.58 & 99.96 & 97.85 & 99.03 & \colorbox{blue!15}{99.05} & \colorbox{blue!35}{99.97} & 97.67 & 98.52 & \colorbox{blue!35}{99.06} & \colorbox{blue!35}{99.98} & 97.62 & 98.60 \\
\bottomrule 
\end{tabular}
}

\label{tab:in_species}
\end{table*}

==> tables/table_traits_manual.tex <==
\begin{table*}[!ht]
\centering
\caption{Trait identification results on the challenging \textbf{manual-annotation test set}. Results are color-coded as \colorbox{blue!35}{Best}, \colorbox{blue!15}{Second best}, \colorbox{red!35}{Worst}, \colorbox{red!15}{Second worst}.
}
\renewcommand{\arraystretch}{0.9}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccccc}
\toprule
\multirow{2}{*}{{Model}} & \multicolumn{5}{c}{{Average Precision}}                                                                          & \multicolumn{4}{c}{{F1@0.5}} & \multicolumn{4}{c}{{F1@optimal threshold}} \\ 
\cmidrule(lr){2-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
 & mAP & Adip & Pelv & Barb & Dors & Adip & Pelv & Barb & Dors & Adip & Pelv & Barb & Dors \\ 
 \midrule
VGG-19 & 38.48 & 49.36 & 23.15 & 35.79 & \colorbox{red!15}{45.61} & 64.89 & 58.48 & 62.53 & 64.09 & 70.12 & 59.19 & 66.48 & 65.87 \\
ResNet-18 & 39.61 & 46.24 & 18.42 & 42.02 & 51.74 & 58.86 & 57.21 & 68.76 & \colorbox{red!15}{59.42} & 69.07 & 57.69 & 70.89 & 66.68 \\
ResNet-34 & 45.53 & 58.78 & 25.66 & 38.66 & 59.02 & 75.17 & 61.16 & 66.45 & 70.64 & 74.81 & 56.85 & 66.9 & 68.02 \\
Inception-v3 & \colorbox{red!35}{30.07} & 48.07 & \colorbox{red!15}{14.22}   & \colorbox{red!35}{22.66} & \colorbox{red!35}{35.32} & 58.86 & \colorbox{red!35}{49.07} & \colorbox{red!35}{58.26} & \colorbox{red!35}{53.36} & 72.76 & \colorbox{red!35}{48.09} & \colorbox{red!15}{60.23} & \colorbox{red!35}{55.66} \\
ResNext-50 & 43.25 & 57.02 & 19.56 & 36.62 & 59.79 & 70.12 & \colorbox{red!15}{52.37} & 63.25 & 62.53 & 73.58 & 52.37 & 62.67 & 68.89 \\
% MobileNet-v3 & 41.99 & 46.18 & 27.96 & 30.44 & 63.36 & 69.87 & 57.63 & 61.03 & 70.68 & 70.5 & 56.75 & 61.72 & 71.85 \\
RegNet-y & 38.1 & 43.45 & 23.14 & 31.93 & 53.87 & 66.74 & 54.87 & 64.19 & 66.65 & 70.37 & \colorbox{red!15}{52.25} & 66.74 & 66.56 \\
EfficientNet-v2 & 55.36 & 63.96 & 30.75 & 55.08 & 71.66 & 74.03 & 60.84 & 73.13 & 75.42 & \colorbox{blue!15}{76.35} & 58.07 & 75.28 & 78.06 \\
% ConvNext-Base & 53.96 & 61.27 & 38.19 & 47.55 & 68.84 & 73.39 & 69.59 & 66.03 & 78.68 & 73.5 & 67.52 & 68.63 & 77.02 \\
\midrule
ViT-B-16 & 37.63 & 37.69 & 26.92 & 36.72 & 49.2 & 64.72 & 58.76 & 66.35 & 66.57 & 65.74 & 60.47 & 66.61 & 67.57 \\
ViT-B-32 & 33.7 & \colorbox{red!35}{33.43} & 24.34 & 30.47 & 46.54 & \colorbox{red!35}{58.11} & 60.19 & 60.33 & 63.91 & \colorbox{red!15}{62.28}   & 56.96 & 63.14 & \colorbox{red!15}{65.76} \\
DEiT-distilled & 40.69 & 40.36 & 32.82 & 29.5 & 60.08 & 61.85 & 64.24 & \colorbox{red!15}{58.77} & 69.82 & 67.34 & 61.97 & 64.11 & 70.63 \\
SWIN-B & 44.68 & 40.67 & 35.6 & 36.36 & 66.07 & 64.16 & 62.32 & 67.73 & 74.7 & 68.0 & 60.16 & 68.14 & 76.93 \\ 
SWIN-B-22k & 51.53 & 55.55 & 32.2 & 50.54 & 67.82 & 72.51 & 65.99 & 73.78 & 75.45 & 72.21 & 63.0 & 71.46 & 74.37 \\ \vspace{0.3em}
CVT-13 & 34.76 & \colorbox{red!15}{35.87} & 24.28 & 30.76 & 48.13 & \colorbox{red!15}{58.53} & 53.3 & 59.69 & 63.48 & \colorbox{red!35}{61.84}   & 57.93 & \colorbox{red!35}{59.69} & 67.91 \\ \vspace{0.3em}
Mobile-ViT-xs     & \colorbox{red!15}{30.6} & 39.08 & \colorbox{red!35}{13.7} & \colorbox{red!15}{23.99} & 45.62 & 65.27 & 54.82 & 62.68 & 64.64 & 69.42 & 52.95 & 61.58 & 67.46 \\ \vspace{0.3em}
Mobile-ViT-v2 & 34.89 & 44.5 & 19.84 & 28.45 & 46.78 & 67.61 & 57.85 & 63.99 & 63.17 & 68.33 & 54.95 & 65.63 & 65.83 \\
MaxViT-t & 49.67 & 50.34 & 33.71 & 51.55 & 63.07 & 69.21 & 65.67 & 74.5 & 72.52 & 68.97 & 63.33 & 72.03 & 71.53 \\
% PVT-v2 & 46.42 & 44.53 & 27.7 & 47.75 & 65.71 & 62.68 & 62.42 & 71.54 & 73.56 & 64.08 & 56.96 & 71.45 & 75.24 \\
\midrule
Q2L (R34-22k SH) & 55.84 & 61.67 & 36.8 & 50.44 & \colorbox{blue!15}{74.43} & \colorbox{blue!35}{76.16} & 67.35 & 73.61 & \colorbox{blue!35}{80.07} & 75.23 & 69.25 & 72.76 & \colorbox{blue!35}{79.63} \\
Q2L (R34-22k MH)  & 53.98 & 56.6 & 40.04 & 45.91 & 73.36 & 75.42 & 67.54 & 72.57 & \colorbox{blue!15}{78.9} & 70.93 & 67.88 & 72.18 & 77.8 \\
Q2L (SWIN-22k SH) & 59.39 & 59.18 & 41.65 & 63.46 & 73.28 & 75.74 & 70.83 & \colorbox{blue!35}{79.16} & 78.69 & 74.8 & 70.54 & \colorbox{blue!35}{77.78} & 78.44 \\
Q2L (SWIN-22k MH) & 58.27 & 57.97 & 42.71 & 60.56 & 71.83 & 74.55 & 70.83 & \colorbox{blue!15}{77.89} & 78.18 & 73.52 & 71.46 & \colorbox{blue!15}{77.68} & 75.53 \\ \midrule
\textbf{MTLSwinB} & 77.34 & 74.74 & \colorbox{blue!35}{95.38} & 66.85 & 72.38 & 62.89 & 97.14 & 63.44 & 67.24 & 66.06 & \colorbox{blue!15}{97.26} & 63.55 & 62.59 \\
% \textbf{ProtoMTL (Ours)} & \colorbox{blue!35}{81.67} & 80.03 & 95.14 & \colorbox{blue!35}{75.67} & \colorbox{blue!35}{75.84} & 68.37 & \colorbox{blue!15}{97.26} & 68.16 & 66.03 & 67.69 & \colorbox{blue!15}{97.26} & 70.81 & 64.55 \\
\textbf{AquaDeHi} & \colorbox{blue!15}{78.97} & \colorbox{blue!15}{80.26}  & \colorbox{blue!15}{95.21} & \colorbox{blue!15}{69.94} & 70.47 & 69.44 & 96.99 & 68.09 & 62.09 & 71.17 & \colorbox{blue!15}{97.26} & 66.34 & 58.88 \\
\textbf{AquaDeHi$^\dagger$} & \colorbox{blue!35}{79.53} & \colorbox{blue!35}{83.65} & 95.11 & 68.87 & 70.50 & 75.38 & \colorbox{blue!35}{97.34} & 70.70 & 67.71 & \colorbox{blue!35}{78.60} & \colorbox{blue!35}{97.29} & 70.97 & 66.67 \\
\bottomrule
\end{tabular}%
}

\label{tab:manual}
\end{table*}

==> tables/table_traits_ood.tex <==
\begin{table*}[!ht]
\centering
\caption{Trait identification results on the \textbf{leave-out-species test set}. Results are color-coded as \colorbox{blue!35}{Best}, \colorbox{blue!15}{Second best}, \colorbox{red!35}{Worst}, \colorbox{red!15}{Second worst}.}
\renewcommand{\arraystretch}{0.9}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccccc}
\toprule
\multirow{2}{*}{{Model}} & \multicolumn{5}{c}{{Average Precision}} & \multicolumn{4}{c}{{F1@0.5}} & \multicolumn{4}{c}{{F1@optimal threshold}} \\ 
\cmidrule(lr){2-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
 & mAP & Adip & Pelv & Barb & Dors & Adip & Pelv & Barb & Dors & Adip & Pelv & Barb & Dors \\ 
 \midrule
VGG-19 & 49.97 & 68.42 & 43.36 & 65.47 & 22.62 & 79.93 & 57.35 & 79.55 & 65.03 & 81.18 & 67.52 & 81.05 & 63.5 \\
ResNet-18 & 49.27 & 81.46 & 23.89 & 80.68 & 11.06 & 79.16 & 66.84 & 83.77 & 54.31 & 85.16 & 64.85 & 84.0 & 55.42 \\
ResNet-34 & 52.14 & 79.8 & 37.24 & 75.45 & 16.09 & 86.67 & 58.07 & 82.87 & 55.76 & 86.67 & 69.73 & 82.87 & 55.73 \\
Inception-v3 & \colorbox{red!35}{28.93} & 67.01 & 6.33 & \colorbox{red!35}{27.27} & 15.13 & 73.56 & 55.49 & \colorbox{red!35}{63.14} & 57.37 & 76.53 & 49.61 & \colorbox{red!35}{61.65} & 61.51 \\
ResNext-50 & 53.0 & 91.16 & \colorbox{red!35}{1.42} & 72.86 & 46.56 & 93.28 & 48.29 & 81.23 & 73.4 & 82.29 & \colorbox{red!15}{48.71} & 80.91 & 72.85 \\
% MobileNet-v3 & 53.36 & 89.93 & 21.18 & 60.63 & 41.68 & 89.58 & 60.13 & 77.15 & 71.08 & 90.16 & 61.08 & 74.65 & 73.2 \\
RegNet-y & 34.67 & 67.04 & 12.23 & \colorbox{red!15}{45.17} & 14.24 & 80.03 & 54.01 & \colorbox{red!15}{69.27} & 57.17 & 75.4 & 56.86 & 71.16 & 56.88 \\
EfficientNet-v2 & 83.86 & 95.45 & 88.1 & 83.97 & 67.91 & 95.15 & 84.59 & 86.76 & 79.31 & 92.76 & 87.07 & 82.62 & 79.43 \\
% ConvNext-Base & 79.6 & 96.87 & 73.18 & 85.14 & 63.21 & 96.24 & 84.32 & 88.3 & 74.24 & 96.24 & 77.98 & 88.3 & 78.71 \\
\midrule
ViT-B-16 & 47.27 & 58.54 & 40.13 & 67.6 & 22.82 & \colorbox{red!15}{69.78}   & 66.66 & 70.2 & 62.41 & \colorbox{red!15}{69.27} & 65.89 & 76.86 & 61.87 \\
ViT-B-32 & 35.29 & \colorbox{red!35}{47.21} & 14.49 & 50.29 & 29.17 & \colorbox{red!35}{69.3} & 56.96 & 69.79 & 64.87 & \colorbox{red!35}{62.59}   & 56.1 & \colorbox{red!15}{64.72} & 63.66 \\
DEiT-distilled & 61.74 & 65.19 & 43.15 & 82.55 & 56.07 & 80.14 & 63.26 & 85.71 & 76.08 & 73.5 & 70.35 & 86.78 & 75.87 \\
SWIN-B & 60.22 & 81.1 & 38.66 & 79.96 & 41.15 & 87.02 & 71.63 & 86.15 & 69.24 & 82.11 & 59.69 & 86.87 & 68.83 \\
SWIN-B-22k & 68.18 & 89.0 & 59.52 & 80.03 & 44.18 & 92.04 & 75.96 & 85.03 & 57.88 & 91.5 & 74.77 & 83.88 & 58.25 \\
CVT-13 & \colorbox{red!15}{28.94} & 55.04 & \colorbox{red!15}{1.84} & 48.15 & \colorbox{red!15}{10.73} & 77.28 & \colorbox{red!15}{48.23} & 72.95 & \colorbox{red!15}{52.77} & 69.61 & \colorbox{red!35}{47.13} & 72.95 & 54.55 \\
Mobile-ViT-xs & 34.23 & 55.65 & 13.99 & 58.08 & \colorbox{red!35}{9.2} & 77.36 & 56.12 & 75.46 & \colorbox{red!35}{52.03} & 76.35 & 54.39 & 75.17 & \colorbox{red!35}{52.67} \\
Mobile-ViT-v2 & 33.76 & \colorbox{red!15}{52.62} & 3.74 & 64.05 & 14.63 & 73.59 & \colorbox{red!35}{46.78} & 79.37 & 54.76 & 70.19 & 51.98 & 77.4 & \colorbox{red!15}{53.75} \\
MaxViT-t & 75.42 & 87.18 & 81.3 & 76.03 & 57.15 & 88.61 & 69.04 & 79.62 & 75.05 & 88.21 & 83.98 & 84.27 & 75.63 \\
% PVT-v2 & 60.72 & 83.91 & 9.26 & 89.3 & 60.42 & 80.42 & 56.72 & 88.41 & 78.74 & 79.24 & 49.62 & 90.49 & 76.61 \\
\midrule
Q2L (R34-22k SH) & 79.86 & 92.93 & 67.54 & 89.14 & 69.82 & 88.54 & 85.56 & 86.14 & 70.02 & 92.79 & 88.51 & 90.09 & 78.74 \\
Q2L (R34-22k MH) & 74.64 & 92.5 & 50.37 & 85.21 & 70.47 & 91.04 & 78.74 & 86.84 & 70.83 & 93.48 & 78.74 & 89.0 & 82.07 \\
Q2L (SWIN-22k SH) & 88.41 & 98.61 & 93.06 & 97.3 & 64.65 & \colorbox{blue!15}{97.84} & 92.75 & \colorbox{blue!15}{96.08} & 74.5 & 97.42 & 93.98 & 95.22 & 75.43 \\
Q2L (SWIN-22k MH) & 88.23 & 99.17 & 96.39 & \colorbox{blue!15}{97.62}  & 59.76 & 97.49 & 99.04 & 95.84 & 73.98 & \colorbox{blue!15}{97.84}  & 98.12 & \colorbox{blue!15}{95.84} & 76.69 \\ \midrule
\textbf{MTLSwinB} & 92.71 & 98.41 & \colorbox{blue!35}{99.95} & 95.74 & 76.75 & 97.14 & \colorbox{blue!15}{99.90} & 91.60 & 59.49 & \colorbox{blue!15}{97.87}  & \colorbox{blue!35}{99.97} & 85.14 & 72.57 \\
% \textbf{ProtoMTL (Ours)} & \colorbox{blue!15}{96.02}  & \colorbox{blue!15}{99.46}  & \colorbox{blue!15}{99.95} & 95.67 & \colorbox{blue!15}{89.00}  & 97.18 & 99.87 & 88.24 & \colorbox{blue!15}{84.79} & 97.18 & \colorbox{blue!15}{99.95} & 85.33 & \colorbox{blue!15}{82.76} \\
\textbf{AquaDeHi} & 94.12 & \colorbox{blue!35}{99.96}  & 99.93 & 95.10 & 81.46 & \colorbox{blue!35}{98.59} & 99.74 & 73.74 & 75.93 & \colorbox{blue!35}{97.90}  & 99.84 & 83.56 & 77.08 \\
\textbf{AquaDeHi$^\dagger$} & \colorbox{blue!35}{97.72} & 98.62 & \colorbox{blue!15}{99.95} & \colorbox{blue!35}{99.43} & \colorbox{blue!35}{92.90} & \colorbox{blue!35}{98.59} & \colorbox{blue!35}{99.95} & \colorbox{blue!35}{96.30} & \colorbox{blue!35}{85.45} & \colorbox{blue!35}{97.90} & \colorbox{blue!15}{99.95} & \colorbox{blue!35}{97.06} & \colorbox{blue!35}{89.45}  \\
\bottomrule
\end{tabular}%
}

\label{tab:ood}
\end{table*}

==> tables/traits_in_new.tex <==
\begin{table*}[h]
\centering
\setlength\tabcolsep{4pt} % Tăng khoảng cách cột
\renewcommand{\arraystretch}{1.1}
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \textbf{mAP} & \multicolumn{4}{c}{\textbf{Trait-wise AP}} \\ 
\cmidrule(lr){2-2} \cmidrule(lr){3-6}
 & \textbf{Mean} & \textbf{Adipose} & \textbf{Pelvic} & \textbf{Barbel} & \textbf{Dorsal} \\ 
\midrule
% --- Backbones ---
\textit{Backbones} & & & & & \\
\textbf{ResNeXt-50} \cite{xie2017aggregated} & 91.44 & 98.53 & 74.64 & 97.03 & 95.54 \\
\textbf{Swin-B-22k} \cite{swin} & 95.21 & 98.05 & 86.94 & 97.55 & 98.28 \\
\textbf{MaxViT-T} \cite{maxvit} & 95.49 & 98.33 & 86.44 & 98.88 & 98.30 \\
\midrule

% --- SOTA Multi-label ---
\textit{SOTA Multi-label} & & & & & \\
\textbf{Q2L (Swin-B)} \cite{liu2021query2label} & 98.94 & \colorbox{blue!15}{99.82} & 94.91 & \colorbox{blue!15}{98.94} & \colorbox{blue!35}{99.61} \\
\midrule

% --- Ours ---
\textit{Ours} & & & & & \\
\textbf{MTLSwinB} (Parallel) & \colorbox{blue!35}{99.38} & 99.75 & \colorbox{blue!35}{99.99} & \colorbox{blue!35}{98.47} & \colorbox{blue!15}{99.29} \\
\textbf{ProtoMTL} & \colorbox{blue!15}{99.34} & \colorbox{blue!35}{99.94} & \colorbox{blue!35}{99.97} & 98.26 & 99.18 \\
\textbf{AquaDeHi} (Proposed) & 99.11 & 99.58 & \colorbox{blue!15}{99.96} & 97.85 & 99.03 \\
\bottomrule 
\end{tabular}
}
\caption{Trait identification results (Average Precision in \%) on the in-species test set. \textbf{Q2L} represents Query2Label, a state-of-the-art multi-label classification method. Results are color-coded as \colorbox{blue!35}{Best} and \colorbox{blue!15}{Second best}.}
\label{tab:in-species-test-set}
\end{table*}

==> tables_short/table_classes.tex <==
\begin{table}[]
\centering
\small
\begin{threeparttable}
\caption{Comparison of Classification Performance (in \%). Results Are Color-coded as \colorbox{blue!35}{Best}, \colorbox{blue!15}{Second best}, \colorbox{red!35}{Worst}, and \colorbox{red!15}{Second worst}}
\label{tab:classification}

\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{1.1}

\begin{tabular}{lccccc}
    \toprule
    \multirow{2.1}{*}{{Model}} & \multirow{2.1}{*}{{F1}} & Major & Neutral & Minor & Ultra-R \\
    &  & Acc. & Acc. & Acc. & Acc. \\
    \midrule
    % --- CNNs ---
    VGG-19 \cite{simonyan2014very} & 49.7 & 93.5 & 83.0 & 74.2 & 45.9 \\
    ResNeXt-50 \cite{xie2017aggregated} & 44.4 & 91.4 & 78.3 & 69.8 & 39.1 \\
    RegNetY-4G \cite{radosavovic2020designing} & 43.7 & 89.8 & 77.4 & 68.5 & 38.5 \\
    \midrule
    % --- Transformers ---
    ViT-B16 \cite{ViT} & 48.3 & 88.7 & 82.3 & 73.3 & 43.4 \\
    Swin-B-22k \cite{swin} & 55.1 & 92.6 & 86.2 & 79.6 & 50.4 \\
    MaxViT-T \cite{maxvit} & 57.8 & 94.4 & \colorbox{blue!15}{86.7} & 81.4 & 53.9 \\
    \midrule
    % --- Foundation Models (Linear Probe) ---
    BioCLIP-LP \cite{stevens2024bioclip} & 38.2 & \colorbox{red!15}{75.5} & \colorbox{red!15}{65.2} & 61.3 & 31.1 \\
    CLIP-LP \cite{radford2021learning} & \colorbox{red!15}{25.4} & \colorbox{red!35}{55.9} & \colorbox{red!35}{49.8} & \colorbox{red!15}{46.7} & \colorbox{red!15}{20.9} \\
    DINOv2-LP \cite{oquab2023dinov2} & 53.1 & 89.9 & 78.0 & 76.0 & 47.0 \\
    \midrule
    % --- FGVC Methods ---
    INTR \cite{paul2023simple} & \colorbox{red!35}{6.1} & 92.2 & 73.2 & \colorbox{red!35}{22.6} & \colorbox{red!35}{0.6} \\
    TransFG \cite{he2022transfg} & 50.3 & 94.5 & 86.6 & 75.5 & 45.3 \\
    \midrule
    % --- Ours ---
    MTLSwinB & \colorbox{blue!15}{57.9} & \colorbox{blue!15}{95.2} & \colorbox{blue!35}{89.0} & \colorbox{blue!15}{85.9} & \colorbox{blue!15}{60.5} \\
    % AquaDeHi & 57.5 & 94.9 & \colorbox{blue!15}{89.0} & 84.1 & \colorbox{blue!15}{61.4} \\
    $\FISHER$ & \colorbox{blue!35}{60.8} & \colorbox{blue!35}{95.5} & \colorbox{blue!35}{89.0} & \colorbox{blue!35}{86.2} & \colorbox{blue!35}{63.8} \\
    \bottomrule
\end{tabular}

\end{threeparttable}
\vspace{-1.0em}
\end{table}

==> tables_short/table_seg.tex <==
\begin{table*}[!htbp]
\small
\centering
\caption{Segmentation Performance Comparison (mIoU in \%) including Input Size.\\Results Are Highlighted as \colorbox{blue!35}{Best}, \colorbox{blue!15}{Second best}, \& \colorbox{red!35}{Worst} (excluding Zero-Shot)}
\setlength\tabcolsep{2.5pt}
\renewcommand{\arraystretch}{1.1}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multirow{2.5}{*}{Model} & \multirow{2.5}{*}{Size} & \multirow{2.5}{*}{mIoU} & \multicolumn{10}{c}{Trait-wise IoU} \\
\cmidrule(lr){4-13}
 & & & \textit{BG} & \textit{Head}  & \textit{Eye} & \textit{Dorsal} & \textit{Pect.} & \textit{Pelvic} & \textit{Anal} & \textit{Caudal} & \textit{Adip.} & \textit{Barbel} \\
    \midrule
    % --- Representative Seg Models ---
    PSPNet \cite{zhao2017pspnet} & \multirow{4}{*}{\textbf{$320\times320$}} & \colorbox{red!35}{73.8} & \colorbox{red!35}{94.6} & \colorbox{red!35}{84.3} & \colorbox{red!35}{77.7} & \colorbox{red!35}{85.1} & \colorbox{red!35}{67.1} & 80.5 & \colorbox{red!35}{83.0} & \colorbox{red!35}{88.7} & \colorbox{red!35}{56.9} & 20.1 \\ 
    DeepLabV3+ \cite{deeplabv3plus2018} &  & 77.0 & 95.4 & 86.0 & 79.1 & 88.1 & 71.0 & \colorbox{blue!35}{84.7} & 86.2 & 89.9 & 66.1 & 23.7 \\ 
    Mask2Former \cite{cheng2021per}&  & \colorbox{blue!15}{81.6} & 95.5 & 86.4 & 79.1 & 87.6 & 74.2 & \colorbox{red!35}{76.1} & 84.7 & 88.8 & 59.6 & \colorbox{red!35}{0.0} \\ 
    YOLOv8 \cite{varghese2024yolov8} &  & \colorbox{blue!35}{83.1} & \colorbox{blue!15}{96.8} & 84.5 & 83.1 & 88.0 & \colorbox{blue!35}{78.0} & 77.5 & 85.6 & 89.6 & 66.8 & 26.7 \\ 
    \midrule
    % --- Our Baseline ---
    MTLSwinB & \textbf{$224\times224$} & 80.4 & 96.7 & 87.8 & 82.7 & 91.5 & 73.5 & 82.9 & 88.5 & \colorbox{blue!15}{92.9} & \colorbox{blue!35}{72.7} & \colorbox{blue!15}{34.5} \\ \midrule
    
    \multirow{2}{*}{$\FISHER$} & \textbf{$224\times224$} & 79.8 & \colorbox{blue!15}{96.8} & \colorbox{blue!15}{88.3} & \colorbox{blue!15}{83.2} & \colorbox{blue!15}{91.6} & 74.0 & 83.0 & \colorbox{blue!15}{89.0} & \colorbox{blue!15}{92.9} & 66.8 & 32.9 \\
      
     & $320\times320$ & 81.4 & \colorbox{blue!35}{97.0} & \colorbox{blue!35}{88.9} & \colorbox{blue!35}{85.8} & \colorbox{blue!35}{92.4} & \colorbox{blue!15}{76.5} & \colorbox{blue!15}{84.3} & \colorbox{blue!35}{89.4} & \colorbox{blue!35}{93.3} & \colorbox{blue!15}{69.7} & \colorbox{blue!35}{36.3} \\
    \midrule
    % --- Zero-shot ---
    MOLMO + SAM \cite{deitke2024molmo} & - & 39.1 & 85.3 & 37.4 & 29.8 & 50.3 & 29.7 & 38.5 & 36.1 & 83.4 & 0.4 & 0.6 \\ 
    \bottomrule
\end{tabular}
}
\label{tab:segmentation}
\vspace{-1.0em}
\end{table*}

==> tables_short/table_traits_inspecies.tex <==
\begin{table*}[h]
\centering
\caption{Trait Identification Results on In-species Test Set (highlighted as \colorbox{blue!35}{Best}, \colorbox{blue!15}{Second best}, \colorbox{red!35}{Worst}, \colorbox{red!15}{Second worst})}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lccccccccccccc}
\toprule
\multirow{2.5}{*}{{Model}} & \multicolumn{5}{c}{{Average Precision}} & \multicolumn{4}{c}{{F1@0.5}} & \multicolumn{4}{c}{{F1@optimal threshold}} \\ 
\cmidrule(lr){2-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
 & mAP & Adip & Pelv & Barb & Dors & Adip & Pelv & Barb & Dors & Adip & Pelv & Barb & Dors \\ \midrule
% --- Representative CNNs ---
ResNext-50 & \csw{91.44} & 98.53 & \csw{74.64} & \csw{97.03} & \csw{95.54} & 96.07 & 86.56 & 96.32 & \csw{94.09} & 96.90 & \csw{85.23} & 96.45 & \csw{94.99} \\
ConvNext-Base & 97.46 & 99.54 & 92.33 & \cs{98.67} & \cs{99.32} & 98.62 & 92.31 & \cb{98.28} & 98.46 & 98.62 & 95.93 & \cb{98.19} & 98.45 \\
\midrule
% --- Representative ViTs ---
ViT-B-16 & \cw{86.95} & \cw{92.93} & \cw{67.70} & \cw{93.29} & \cw{93.89} & \cw{91.51} & \cw{66.75} & \cw{92.41} & \cw{92.57} & \cw{91.71} & \cw{81.23} & \cw{92.14} & \cw{92.68} \\
SWIN-B-22k & 95.21 & \csw{98.05} & 86.94 & 97.55 & 98.28 & \csw{95.95} & \csw{86.37} & \csw{96.07} & 96.47 & \csw{96.12} & 91.29 & \csw{96.13} & 96.62 \\
\midrule
% --- SOTA Competitor ---
Q2L (R34-22k SH) & 97.78 & 99.47 & 93.91 & 98.47 & 99.26 & 97.65 & 97.36 & 97.35 & 98.27 & 97.90 & 95.10 & 97.73 & 98.45 \\
Q2L (SwinB-22k SH) & 98.32 & \cb{99.81} & 94.94 & \cb{99.00} & \cb{99.53} & \cb{99.09} & 97.36 & \cs{97.82} & \cb{99.19} & \cs{98.93} & 95.66 & \cs{98.03} & \cb{99.06} \\
\midrule
% --- Proposed Methods ---
MTLSwinB & \cb{99.38} & \cs{99.75} & \cb{99.99} & 98.47 & 99.29 & 98.57 & \cb{99.97} & 97.19 & 98.21 & 98.87 & \cs{99.97} & 97.15 & 98.43 \\
$\FISHER$  & \cs{99.11} & 99.58 & \cs{99.96} & 97.85 & 99.03 & \cs{99.05} & \cb{99.97} & 97.67 & \cs{98.52} & \cb{99.06} & \cb{99.98} & 97.62 & \cs{98.60} \\
\bottomrule 
\end{tabular}
}
\label{tab:in_species}
\vspace{-0.5em}
\end{table*}

==> tables_short/table_traits_manual.tex <==
\begin{table*}[!ht]
\centering
\caption{Trait Identification Results on Manual-annotation Test Set (highlighted as \colorbox{blue!35}{Best}, \colorbox{blue!15}{Second best}, \colorbox{red!35}{Worst}, \colorbox{red!15}{Second worst})}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lccccccccccccc}
\toprule
\multirow{2.5}{*}{{Model}} & \multicolumn{5}{c}{{Average Precision}} & \multicolumn{4}{c}{{F1@0.5}} & \multicolumn{4}{c}{{F1@optimal threshold}} \\ 
\cmidrule(lr){2-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
 & mAP & Adip & Pelv & Barb & Dors & Adip & Pelv & Barb & Dors & Adip & Pelv & Barb & Dors \\ 
 \midrule
% --- Representative CNNs ---
ResNext-50 & \colorbox{red!15}{43.25} & 57.02 & \colorbox{red!35}{19.56} & \colorbox{red!35}{36.62} & \colorbox{red!15}{59.79} & 70.12 & \colorbox{red!35}{52.37} & \colorbox{red!35}{63.25} & \colorbox{red!35}{62.53} & 73.58 & \colorbox{red!35}{52.37} & \colorbox{red!35}{62.67} & 68.89 \\
% --- Representative ViTs ---
ViT-B-16 & \colorbox{red!35}{37.63} & \colorbox{red!35}{37.69} & \colorbox{red!15}{26.92} & \colorbox{red!15}{36.72} & \colorbox{red!35}{49.20} & \colorbox{red!15}{64.72} & \colorbox{red!15}{58.76} & 66.35 & \colorbox{red!15}{66.57} & \colorbox{red!35}{65.74} & \colorbox{red!15}{60.47} & 66.61 & 67.57 \\
SWIN-B-22k & 51.53 & \colorbox{red!15}{55.55} & 32.20 & 50.54 & 67.82 & 72.51 & 65.99 & \colorbox{blue!15}{73.78} & 75.45 & 72.21 & 63.00 & 71.46 & 74.37 \\ 
\midrule
% --- SOTA Competitor ---
Q2L (R34-22k SH) & 55.84 & 61.67 & 36.80 & 50.44 & \colorbox{blue!35}{74.43} & \colorbox{blue!35}{76.16} & 67.35 & 73.61 & \colorbox{blue!35}{80.07} & \colorbox{blue!15}{75.23} & 69.25 & \colorbox{blue!15}{72.76} & \colorbox{blue!35}{79.63} \\
Q2L (SWIN-22k SH) & 59.39 & 59.18 & 41.65 & 63.46 & \colorbox{blue!15}{73.28} & \colorbox{blue!15}{75.74} & 70.83 & \colorbox{blue!35}{79.16} & \colorbox{blue!15}{78.69} & 74.80 & 70.54 & \colorbox{blue!35}{77.78} & \colorbox{blue!15}{78.44} \\
\midrule
% --- Proposed Methods ---
MTLSwinB & \colorbox{blue!15}{77.34} & \colorbox{blue!15}{74.74} & \colorbox{blue!35}{95.38} & \colorbox{blue!15}{66.85} & 72.38 & \colorbox{red!35}{62.89} & \colorbox{blue!15}{97.14} & \colorbox{red!15}{63.44} & 67.24 & \colorbox{red!15}{66.06} & \colorbox{blue!15}{97.26} & \colorbox{red!15}{63.55} & \colorbox{red!35}{62.59} \\
% AquaDeHi & \colorbox{blue!15}{78.97} & \colorbox{blue!15}{80.26} & \colorbox{blue!15}{95.21} & \colorbox{blue!35}{69.94} & 70.47 & 69.44 & 96.99 & 68.09 & \colorbox{red!35}{62.09} & 71.17 & \colorbox{blue!15}{97.26} & 66.34 & \colorbox{red!35}{58.88} \\
$\FISHER$ & \colorbox{blue!35}{79.53} & \colorbox{blue!35}{83.65} & \colorbox{blue!15}{95.11} & \colorbox{blue!35}{68.87} & 70.50 & 75.38 & \colorbox{blue!35}{97.34} & 70.70 & 67.71 & \colorbox{blue!35}{78.60} & \colorbox{blue!35}{97.29} & 70.97 & \colorbox{red!15}{66.67} \\
\bottomrule
\end{tabular}%
} \vspace{-1em}
\label{tab:manual}
\end{table*}

==> tables_short/table_traits_ood.tex <==
\begin{table*}[!ht]
\centering
\caption{Trait Identification Results on Leave-out-species Test Set (highlighted as \colorbox{blue!35}{Best}, \colorbox{blue!15}{Second best}, \colorbox{red!35}{Worst}, \colorbox{red!15}{Second worst})}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lccccccccccccc}
\toprule
\multirow{2.5}{*}{{Model}} & \multicolumn{5}{c}{{Average Precision}} & \multicolumn{4}{c}{{F1@0.5}} & \multicolumn{4}{c}{{F1@optimal threshold}} \\ 
\cmidrule(lr){2-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
 & mAP & Adip & Pelv & Barb & Dors & Adip & Pelv & Barb & Dors & Adip & Pelv & Barb & Dors \\ 
 \midrule
% --- Representative CNNs ---
ResNext-50 & \colorbox{red!15}{53.00} & 91.16 & \colorbox{red!35}{1.42} & \colorbox{red!15}{72.86} & 46.56 & 93.28 & \colorbox{red!35}{48.29} & \colorbox{red!15}{81.23} & 73.40 & \colorbox{red!15}{82.29} & \colorbox{red!35}{48.71} & \colorbox{red!15}{80.91} & 72.85 \\
% --- Representative ViTs ---
ViT-B-16 & \colorbox{red!35}{47.27} & \colorbox{red!35}{58.54} & \colorbox{red!15}{40.13} & \colorbox{red!35}{67.60} & \colorbox{red!35}{22.82} & \colorbox{red!35}{69.78} & \colorbox{red!15}{66.66} & \colorbox{red!35}{70.20} & 62.41 & \colorbox{red!35}{69.27} & \colorbox{red!15}{65.89} & \colorbox{red!35}{76.86} & \colorbox{red!15}{61.87} \\
SWIN-B-22k & 68.18 & \colorbox{red!15}{89.00} & 59.52 & 80.03 & \colorbox{red!15}{44.18} & 92.04 & 75.96 & 85.03 & \colorbox{red!35}{57.88} & 91.50 & 74.77 & 83.88 & \colorbox{red!35}{58.25} \\
\midrule
% --- SOTA Competitor ---
Q2L (R34-22k SH) & 79.86 & 92.93 & 67.54 & 89.14 & 69.82 & \colorbox{red!15}{88.54} & 85.56 & 86.14 & 70.02 & 92.79 & 88.51 & 90.09 & \colorbox{blue!15}{78.74} \\
Q2L (SWIN-22k SH) & 88.41 & \colorbox{blue!15}{98.61} & \colorbox{blue!15}{93.06} & \colorbox{blue!15}{97.30} & 64.65 & \colorbox{blue!15}{97.84} & 92.75 & \colorbox{blue!15}{96.08} & \colorbox{blue!15}{74.50} & 97.42 & 93.98 & \colorbox{blue!15}{95.22} & 75.43 \\
\midrule
% --- Proposed Methods ---
MTLSwinB & \colorbox{blue!15}{92.71} & 98.41 & \colorbox{blue!35}{99.95} & 95.74 & \colorbox{blue!15}{76.75} & 97.14 & \colorbox{blue!15}{99.90} & 91.60 & \colorbox{red!15}{59.49} & \colorbox{blue!15}{97.87} & \colorbox{blue!35}{99.97} & 85.14 & 72.57 \\
% AquaDeHi & \colorbox{blue!15}{94.12} & \colorbox{blue!35}{99.96} & \colorbox{blue!15}{99.93} & 95.10 & \colorbox{blue!15}{81.46} & \colorbox{blue!35}{98.59} & 99.74 & \colorbox{red!15}{73.74} & \colorbox{blue!15}{75.93} & \colorbox{blue!35}{97.90} & 99.84 & 83.56 & 77.08 \\
$\FISHER$ & \colorbox{blue!35}{97.72} & \colorbox{blue!35}{98.62} & \colorbox{blue!35}{99.95} & \colorbox{blue!35}{99.43} & \colorbox{blue!35}{92.90} & \colorbox{blue!35}{98.59} & \colorbox{blue!35}{99.95} & \colorbox{blue!35}{96.30} & \colorbox{blue!35}{85.45} & \colorbox{blue!35}{97.90} & \colorbox{blue!15}{99.95} & \colorbox{blue!35}{97.06} & \colorbox{blue!35}{89.45} \\
\bottomrule
\end{tabular}%
}
\label{tab:ood}
\vspace{-0.5em}
\end{table*}
